Context Conquers Parameters: Outperforming Proprietary LLM in Commit Message Generation

Commit messages provide descriptions of the modifications made in a commit using natural language, making them crucial for software maintenance and evolution. Recent developments in Large Language Models (LLMs) have led to their use in generating high-quality commit messages, such as the Omniscient Message Generator (OMG). This method employs GPT-4 to produce state-of-the-art commit messages. However, the use of proprietary LLMs like GPT-4 in coding tasks raises privacy and sustainability concerns, which may hinder their industrial adoption. Considering that open-source LLMs have achieved competitive performance in developer tasks such as compiler validation, this study investigates whether they can be used to generate commit messages that are comparable with OMG. Our experiments show that an open-source LLM can generate commit messages that are comparable to those produced by OMG. In addition, through a series of contextual refinements, we propose lOcal MessagE GenerAtor (OMEGA) , a CMG approach that uses a 4-bit quantized 8B open-source LLM. OMEGA produces state-of-the-art commit messages, surpassing the performance of GPT-4 in practitioners' preference.

==> Sections/implications.tex <==

\subsection{For Researchers}
Our study demonstrates that high-quality CM can be generated using an SLM through a series of commit context enhancements. 
This finding encourages researchers to explore ways to carefully curate task-specific contextual information provided to an LLM to achieve superior results, rather than relying solely on larger proprietary LLMs with poorly devised context.
% This finding opens up new avenues for research in the field of software engineering, particularly in the application of smaller, more efficient models for complex tasks. 
% Researchers can build on our work by exploring additional enhancements to commit context, such as incorporating more detailed code analysis or leveraging additional types of contextual information. 
Furthermore, our proposed FIDEX presents a novel approach to summarizing code changes, which can be extended and refined for other software engineering tasks in which code-changes play a pivotal role \cite{fan2024exploringcapabilitiesllmscode}. By showing that a quantized instruction-tuned Llama3 model with 8B trained parameters can outperform GPT-4 in the CMG task, we encourage further exploration of smaller, cost-effective models in various software engineering tasks.

\subsection{For Industry}

Our approach to generating high-quality CM using an SLM offers significant advantages for the industry. The quantized instruction-tuned Llama3 model with 8B trained parameters can be deployed on a GPU with 8GB of VRAM, making it accessible for companies and practitioners with limited computational resources. This model can be deployed on local hardware, ensuring that high-quality CM can be generated without incurring substantial costs associated with proprietary models like GPT-4. Furthermore, using an open-source LLM enhances data privacy, as companies can avoid sharing sensitive code with external providers. 
% By adopting our superior CMG approach, organizations can high-quality CMs, improving software maintenance and evolution \cite{li2021commitmessagematters}, while maintaining cost efficiency and data confidentiality.


